Execution-Time Opacity in (Controllable) Timed Automata is Hard

Timing information leakage occurs whenever an attacker successfully deduces confidential internal information by observing some timed information such as the total duration of a run. Timed automata (TAs) are an extension of finite-state automata with a set of clocks evolving at the same rate and that can be tested or reset. Hence, this formalism is able to represent systems involving timing constraints reacting to the passage of time. Some of the transitions in a timed automaton may be controlled, i.e., enabled or disabled, to limit the runs that are allowed. Execution-time opacity (ET-opacity) aims at studying timing information leakage through the analysis of timed automata. More precisely, the ET-opacity problem consists in deciding whether an attacker can deduce whether some secret locations were visited by a run, solely from the run's duration. When control is allowed, the goal becomes to find a strategy that blocks the runs leaking information. This problem has been shown decidable for TAs, with and without control. However, these existing results only provide upper bounds on the complexity of the ET-opacity problem, sometimes largely above the tight bound. Our main contribution is to provide tight lower bounds for those two results. Moreover, for controllable TAs, two variants of ET-opacity (depending on whether detecting if a run did not visit a secret location represents an information leakage or not, and named full and weak ET-opacity respectively) had been separately studied; we prove here that these two notions are inter-reducible.

==> eptcsdata.tex <==
\providecommand{\firstpage}{84}
\providecommand{\publicationstatus}{G. Bacci, M. Randour (Eds.): Seventeenth\\
International Symposium on Games, Automata, Logics,\\
and Formal Verification (GandALF 2026)\\
EPTCS 454, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.454.7}{10.4204/EPTCS.454.7}}

